Rehabilitating CIV-based black hole mass estimates in quasars

Currently, the ability to produce black hole mass estimates using the CIV 1549 line that are consistent with Hb mass estimates is uncertain, due in large part to disagreement between velocity line width measurements for the two lines. This discrepancy between Hb and CIV arises from the fact that both line profiles are treated the same way in single-epoch scaling relationships based on the assumption that the broad-line region is virialized, even though a non-virialized emission component is often significant in the CIV line and absent or weak in the Hb line. Using quasi-simultaneous optical and ultra-violet spectra for a sample of 85 optically bright quasars with redshifts in the range z=0.03-1.4, we present a significant step along the path to rehabilitating the CIV line for black hole mass estimates. We show that the residuals of velocity line width between CIV and Hb are significantly correlated with the peak flux ratio of SiIV+OIV] 1400 to CIV. Using this relationship, we develop a prescription for estimating black hole masses from the ultra-violet spectrum that agree better with Hb-based masses than the traditional CIV masses. The scatter between Hb and CIV masses is initially 0.43 dex in our sample and is reduced to 0.33 dex when using our prescription. The peak flux ratio of SiIV+OIV] 1400 to CIV is an ultraviolet indicator of the suite of spectral properties commonly known as "Eigenvector 1", thus the reduction in scatter between CIV and Hb black hole masses is essentially due to removing an Eigenvector 1 bias in CIV-based masses.

==> correlations.tex <==
\begin{table*}
\begin{minipage}{13cm}
\renewcommand{\thefootnote}{\alph{footnote}}
\caption{Correlations \label{tab:correlation}}
\begin{tabular}{llcrr}
Param 1 & Param 2 & N & $\rho$ \footnotemark[1]   & P \footnotemark[2]      \\
\hline
 $\Delta$log(FWHM)(\CIV$-$\Hb) & log(\siivoiv\,Peak/\CIV\,Peak) & 39 & $   0.000$ & $   0.000$ \\
 log(\FeII\,EW/\OIII\,EW) & log(\siivoiv\,Peak/\CIV\,Peak) & 39 & $   0.000$ & $   0.000$ \\
\hline
\end{tabular}
\footnotetext[1]{$\rho$ is the Spearman rank correlation coefficient.}
\footnotetext[2]{P is the given probability that the observed distribution of points would arise by chance.}
\end{minipage}
\end{table*}

